Sparse is Enough in Scaling Transformers

Large Transformer models yield impressive results on many tasks, but are expensive to train, or even fine-tune, and so slow at decoding that their use and study becomes out of reach. We address this problem by leveraging sparsity. We study sparse variants for all layers in the Transformer and propose Scaling Transformers, a family of next generation Transformer models that use sparse layers to scale efficiently and perform unbatched decoding much faster than the standard Transformer as we scale up the model size. Surprisingly, the sparse layers are enough to obtain the same perplexity as the standard Transformer with the same number of parameters. We also integrate with prior sparsity approaches to attention and enable fast inference on long sequences even with limited memory. This results in performance competitive to the state-of-the-art on long text summarization.

==> recurrence.tex <==
\section{Recurrence}
[Lukasz]: write

[STRETCH]: add a point about layer repetition

NEW for 250k
baseline, PPL=1.710
SRU=(1,32), PPL=1.684

% \section{Fine-tuning on CPU at home}
% Why: In abstract we mention that it is possible to finetune on CPU. How do we want to do this?

% Problem with Sparse FeedForward here: This probably require processing example by example; then we can probably use modified sparse feedforward... However, with pretraining on multiple tokens we will likely hit all weights in every layer. Assuming uniform distribution with 512 tokens and sparsity 64, we hit each single block in SparseFFL 8 times on average, so very few of them will be skipped. If the distribution is highly nonuniform/spike then we're good (but if that's the case we should consider pruning those blocks altogether, maybe?)

